Gaussian Switch Sampling: A Second Order Approach to Active Learning

In active learning, acquisition functions define informativeness directly on the representation position within the model manifold. However, for most machine learning models (in particular neural networks) this representation is not fixed due to the training pool fluctuations in between active learning rounds. Therefore, several popular strategies are sensitive to experiment parameters (e.g. architecture) and do not consider model robustness to out-of-distribution settings. To alleviate this issue, we propose a grounded second-order definition of information content and sample importance within the context of active learning. Specifically, we define importance by how often a neural network "forgets" a sample during training - artifacts of second order representation shifts. We show that our definition produces highly accurate importance scores even when the model representations are constrained by the lack of training data. Motivated by our analysis, we develop Gaussian Switch Sampling (GauSS). We show that GauSS is setup agnostic and robust to anomalous distributions with exhaustive experiments on three in-distribution benchmarks, three out-of-distribution benchmarks, and three different architectures. We report an improvement of up to 5% when compared against four popular query strategies.

==> sections/IntroductionBACKUP.tex <==
\section{Introduction}

A core factor in the success of machine learning algorithms is the selection of suitable data. While several samples contain valuable information for a given task, other samples may be redundant with little additional information or anomalous with contradicting features. Active Learning~\cite{cohn1996active} is a paradigm in machine learning that tackles this issue by iteratively selecting the most informative samples from a large unlabelled data pool for annotation and training. Due to its intuitive practicality, active learning has already impacted multiple industrial sectors including manufacturing \cite{tong2001active}, robotics \cite{alrobotics}, recommender systems \cite{alrecommender}, medical imaging \cite{hoi2006batch}, and autonomous vehicles \cite{haussmann2020scalable}.
	
At the core of every active learning approach stands its method to select the next set of annotation samples - its acquisition function. Typically, the acquisition function establishes a ranking based on the \emph{importance} of unlabeled samples and interactively selects the next batch based on the prior ordering. Therefore, the acquisition functions typically differ by the manner in which \emph{importance} is defined and how data is selected based on the prior definition of importance. Overall, there are two simple intuitive approaches that form the basis of active learning acquisition functions. The first approach establishes the ordering/sampling method based on generalization difficulty \cite{roth2006margin, wang2014new, gal2017deep, houlsby2011bayesian}. For instance, the most "informative" samples could be underrepresented classes or difficult samples with overlapping class features. In contrast, the second approach orders samples according to dataset representation \cite{sener2017active, longtailcoreset, gissin2019discriminative}. Intuitively, this branch focuses on finding data subsets that best represent the entire dataset and emphasize data diversity within the acquisition batch. 

Although both approaches follow fundamentally different principles, existing protocols employ similar mechanics to define importance within an active learning setting. Specifically, they define importance on the model representation directly. For instance, entropy sampling \cite{wang2014new} selects samples with the highest softmax entropy of the model and is therefore directly dependent on the logits or sample representation. As another example, coreset sampling \cite{sener2017active} maximizes diversity by constructing the coreset of the sample representations directly. Even though these definitions are intuitive, high representation dependence results in severe challenges that often inhibit the deployment of active learning.\\

The first of these challenges is a model's sensitivity to architecture, dataset, optimizer, and hyperparameter choices. For this reason, we find that existing protocols are not consistent over different setup constellations and performance can severely differ when any component is changed or slightly altered. For instance, our experiments show that several protocols outperform the random selection baseline with one architecture but underperform with another. In practice, a user must therefore pick the ``correct" protocol for the specific application and it is unclear if selecting with a random baseline would render higher results. The second challenge in using representation-dependent definition of informativeness is that model representations are sensitive to unknown inputs \cite{hendrycks2019robustness, Temel2017_NIPSW}. A model's performance is severely affected if it is exposed to distributions it was not trained on~\cite{kwon2019distorted, prabhushankar2021contrastive}. We refer to such samples as being out-of-distribution (OOD). As a toy example, consider a model that is exposed to aberrant samples during deployment (Figure~\ref{fig:ood-toy}). Two different protocols may result in similar in-distribution test performance but one strategy may select more aberrant training samples resulting in a more robust model representation. Even though out-of-distribution performance is inherently relevant for active learning, existing protocols do not consider performance on different distributions.

\begin{figure}[!h]
    \begin{center}
        %\hspace*{-1.9cm}
        \includegraphics[scale=0.37]{Fig/ood-toy.png}
    \end{center}
    \caption{Toy example of out-of-distribution performance in active learning. Both protocols result in similar test performance but severely differ when deployed on out-of-distribution samples.}
    \label{fig:ood-toy}
\end{figure}

In this paper, we approach this problem by viewing sample importance as shifts within the data manifold. Specifically, we define ``informativeness" by approximating the frequency in which a model ``forgets" unlabeled samples during training. By effectively counting decision boundary shifts we naturally alleviate the direct representation dependence. We find that our definition not only results in robust importance scores but further find that our scores are exceptionally accurate that can even result in bias towards anomalous samples if deployed directly as an active learning protocol. For this purpose, we combine our definition with an interactive mixture model and develop Gaussian Switch Sampling or \texttt{GauSS} in short. We validate our algorithm with exhaustive experiments and compare against popular protocols used in practical active learning pipelines. Overall, we find that \texttt{GauSS} is robust to setup changes, performs favorably in out-of-distribution settings, and achieves up to 5\% improvement in terms of accuracy. 

%The first is the reliance on accurate data representations. The success of an active learning algorithm depends on the ability to accurately measure the sample position on a global scale in a setup independent fashion. In other words, we need to ensure fixed representations  regardless of the training setup and training pool size. However, in practical machine learning pipelines logit coordinates are not agnostic and representations depend on a variety of parameter choices and random factors (architecture, learning rate, initialization etc.). The second is the lacking evaluation clarity in existing strategies. Specifically, query strategy performance may not be apparent in common numerical evaluation metrics (e.g. class accuracy) and can be dictated by the target task. For instance, uncertainty based strategies could improve the accuracy on aberrant samples while representative strategies outperform on structural characteristics. Both approaches may improve the overall accuracy by the same margin but can result in fundamentally different models with contradicting behavior. For this reason, popular strategies frequently perform radically different depending on the training setup or design choices. This is especially troubling in safety-critical applications (e.g. autonomous vehicles), where explainable and predictable behavior is conditional for successful deployment \cite{Temel2017_NIPSW, temel2019traffic}. In this paper, we address this problem by providing two important contributions: 

%First, we introduce a setup independent measure of the sample position within the representation space. We do so by leveraging a setup robust uncertainty definition for active learning protocols. Similar to existing strategies, we define uncertainty with decision boundary proximity. However, in addition to setup specific uncertainty factors, we further integrate data interaction characteristics that are model and setup independent. This is fundamentally different to existing definitions that base active learning uncertainty on model dependent features exclusively \cite{gissin2019discriminative, gal2017deep, kendall2017uncertainties, houlsby2011bayesian, roth2006margin, wang2014new}. Intuitively, we reason that uncertainty of an arbitrary sample manifests in the learning difficulty of a sample and that uncertain samples are more difficult to learn than less uncertain samples. Following this intuition, we measure learning difficulty by tracking how often samples are "forgotten" during training. We show the gravity of this approach in Figure~\ref{fig:ideal-div-unc}. In this experiment, we establish a query strategy ordering based on the most forgotten and least forgotten samples in the training set and perform active learning on the CIFAR10 dataset. The most uncertain samples are the most difficult to learn but contain the most information. This results in low accuracy values in early rounds but in outperformance in later rounds. In contrast, least uncertain samples are learnt quickly and contain valuable information for frequently appearing features. However, they do not contain a significant amount of additional information which results in an accuracy stagnation until other samples are added. Our observations are complimentary to \cite{toneva2018empirical} where frequently "forgotten" samples are regarded as approximated support vectors within the dataset.

%As a second contribution, we develop a setup-agnostic active learning strategy that produces stable state-of-the-art performance over numerous training settings. Similar to our previous uncertainty definition, our method is based on learning dynamics in neural networks. However, since labels are required to determine if a sample was "forgotten", we approximate uncertainty on the unlabeled pool with prediction switches. Combined with an interactive gaussian sampling technique, our method queries both uncertain and representative samples within a dataset. In addition to common metrics, we further evaluate our approach on out-of-distribution benchmarks as well as partitioned test sets that exhibit different uncertainty properties. We show that our approach matches or outperforms state-of-the-art along all of the above and further shows setup-agnosticity with different architecture, optimizer and hyperparameter choices.

%\begin{enumerate}
%    \item We provide a unifying definition of uncertainty and diversity for active learning based on neural network "forgetting". To the best of our knowledge, this is the first paper that provides a portable definition applicable to any active learning protocol involving neural networks.
%    \item We deploy "forgetting" statistics to differentiate and analyze model interactions with uncertain/diverse samples separately. Our method exposes weaknesses within model manifolds and allows us to critically analyze active learning protocols.
%    \item Based on our empirical findings, we develop Gaussian Switch Sampling (GauSS) - a learning dynamics-based active learning approach. GauSS matches or outperforms existing state-of-the-art strategies while maintaining robustness qualities on out-of-distribution data. 
%\end{enumerate}

%\begin{figure*}[!th]
%    \begin{center}
%        \includegraphics[scale=0.42]{Fig/ideal-uncertainty-and-diversity.png}
%    \end{center}
%    \caption{Example of active learning with most forgotten as well as least forgotten samples. Left shows the most most/least uncertain samples queried by the strategy ordering and the right shows the corresponding active learning curves in comparison to the random baseline. The importance rankings (forgetting frequency) of both strategies are derived from a ResNet18 network.}
%    \label{fig:ideal-div-unc}
%\end{figure*}

==> sections/tmp.tex <==
\begin{table*}[!h]
	\centering
	\begin{tabular}{ |p{0.2cm}|p{1.9cm}||p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|}
		\hline
		\multicolumn{2}{|c||}{}   & \multicolumn{3}{|c|}{Out-Of-Distr.} & \multicolumn{3}{|c|}{In-Distr.} \\
		\hline
		
		\multicolumn{1}{|c|}{} & \multicolumn{1}{|c||}{Algorithms} & \multicolumn{1}{|c|}{CIFAR10-C}  & \multicolumn{1}{|c|}{CINIC10}  & \multicolumn{1}{|c|}{STL10} & \multicolumn{1}{|c|}{CIFAR10} & \multicolumn{1}{|c|}{CINIC10} & \multicolumn{1}{|c|}{CURE-TSR}\\
		\hline
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet-18}}}  	& \bf{GauSS}                      & $\mathbf{17.76}$ & $\mathbf{13.72}$ & $\mathbf{7.17}$                                                                          & $\mathbf{17.77}$ & $\mathbf{17.77}$ & $\mathbf{33.55}$ \\
                                                                        		& ALBL \cite{hsu2015active}       & 10.19            & 5.66             & -4.55            & 7.25             & 7.25             & 22.80              \\
                                                                        		& Coreset \cite{sener2017active}  & -41.87           & -35.07           & -20.58           & -41.04           & 7.25              & -38.60            \\
                                                                        		& Entropy \cite{wang2014new}      & 7.83             & 8.58             & 2.16             & 0.45             & 7.25             & -25.02            \\
                                                                        		& L. Conf. \cite{wang2014new}     & 16.23            & 13.47            & 3.20             & 9.93             & 7.25             & 5.74               \\
                                                                        		\hline
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{DenseNet-121}}}& \bf{GauSS}                      & $\mathbf{13.64}$ & $\mathbf{10.01}$ & $\mathbf{-1.28}$                                                                         & $\mathbf{11.46}$ & $\mathbf{19.30}$ & $\mathbf{19.30}$ \\
                                                                        		& ALBL \cite{hsu2015active}       & 7.69             & 6.67             & -8.56            & 3.28             & 7.25             & 7.25             \\
                                                                        		& Coreset \cite{sener2017active}  & -23.40           & -14.36           & -24.98           & -21.74           & 7.25              & 7.25             \\
                                                                        		& Entropy \cite{wang2014new}      & 1.77             & 2.52             & -10.25             & -7.76            & 7.25             & 7.25             \\
                                                                        		& L. Conf. \cite{wang2014new}     & -0.20            & 3.81             & -11.48           & -3.57            & 7.25             & 7.25             \\
                                                                        		\hline
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet-34}}}  	& \bf{GauSS}                      & $\mathbf{18.14}$ & $\mathbf{16.58}$ & 2.12                                                                                     & $\mathbf{19.30}$ & $\mathbf{19.30}$ & $\mathbf{19.30}$ \\
                                                                        		& ALBL \cite{hsu2015active}       & 7.56             & 9.67             & 0.41             & 13.96            & 7.25             & 7.25             \\
                                                                        		& Coreset \cite{sener2017active}  & -8.25            & -7.18            & -9.23            & -5.21            & 7.25             & 7.25             \\
                                                                        		& Entropy \cite{wang2014new}      & 14.80            & 15.31            & $\mathbf{5.93}$  & 12.51            & 7.25             & 7.25             \\
                                                                        		& L. Conf. \cite{wang2014new}     & 17.52            & 16.60            & 4.91             & 15.99            & 7.25             & 7.25             \\
		\hline
	\end{tabular}
	\caption{Area under difference curve with reference to random sampling over several datasets, query strategies, and architectures. Positive, and higher numbers are better. Negative numbers imply that the strategy has a lower accuracy curve than the random baseline.}
	\label{table:results-overall}
\end{table*}
